Rectangle Coincidences and Sweepouts

We prove an integral formula for continuous paths of rectangles inscribed in a piecewise smooth loop. We then use this integral formula to show that (with a very mild genericity hypothesis) the number of rectangle coincidences, informally described as the number of inscribed rectangles minus the number of isometry classes of inscribed rectangles, grows linearly with the number of positively oriented extremal chords -- a.k.a. diameters -- of the polygon

==> 4lines.tex <==
\section{Four Lines and a Rectangle}

\subsection{The Generic Case}




\end{document}




\newpage

==> 4rectangle.tex <==
\section{Four Rectangles and a Line}

In this chapter we present some of
the results from [{\bf S3\/}] in
abbreviated form.

\subsection{Statement of Results}



